Metric and Kernel Learning using a Linear Transformation

Metric and kernel learning are important in several machine learning applications. However, most existing metric learning algorithms are limited to learning metrics over low-dimensional data, while existing kernel learning algorithms are often limited to the transductive setting and do not generalize to new data points. In this paper, we study metric learning as a problem of learning a linear transformation of the input data. We show that for high-dimensional data, a particular framework for learning a linear transformation of the data based on the LogDet divergence can be efficiently kernelized to learn a metric (or equivalently, a kernel function) over an arbitrarily high dimensional space. We further demonstrate that a wide class of convex loss functions for learning linear transformations can similarly be kernelized, thereby considerably expanding the potential applications of metric learning. We demonstrate our learning approach by applying it to large-scale real world problems in computer vision and text mining.

==> extensions.tex <==
\section{Extensions}\label{sec:ext}
In section~\ref{sec:alg}, we showed that the kernel learning problem could
be computed with respect to a set of basis vectors $\{{\bm x_1}, \ldots,
{\bm x_k}\}$.  


==> formulation.tex <==
\vspace*{-10pt}
\section{Problem Formulation}
\label{sec:prob-formulation}
Given a set of $n$ points $\{\bm{x}_1, ..., \bm{x}_n\}$ in $\mathbb{R}^d$, 
we seek a linear transformation of the data that reflects the provided side-information about the data. In this work, we assume that prior knowledge is known regarding inter-point distances and the goal is to learn a linear transformation of the data so that the Euclidean distance function in the transformed space satisfy the provided inter-point distances. Let $G$ be the learned transformation, then %we parameterizes the Mahalanobis distance. In particular, we learn a positive definite matrix $A$ parameterizing the (squared) Mahalanobis distance.% which parameterizes the (squared) Mahalanobis distance. This in turn parameterizes the (squared) 
\begin{equation}
  \label{eq:1_0}
  \dist (G\bm{x}_i, G\bm{x}_j) = \maha{x}{x},
\end{equation}
where $A=G^TG$ is a positive definite matrix parameterizing the (squared) Mahalanobis distance, i.e.,
\begin{equation}
  \label{eq:1_0}
  \dist_A (\bm{x}_i, \bm{x}_j) = \maha{x}{x},
\end{equation}


%We assume that prior knowledge is known regarding inter-point distances.
We consider relationships constraining the similarity or dissimilarity between
pairs of points.  Two points are similar if the Mahalanobis distance between
them is smaller than a given upper bound, i.e., $\dist (\bm{x}_i, \bm{x}_j)
\leq u$ for a relatively small value of $u$.  Similarly, two points are
dissimilar if $\dist (\bm{x}_i, \bm{x}_j) \geq \ell$ for sufficiently large
$\ell$. Such constraints are typically inputs for many semi-supervised learning
problems, and can also be readily inferred in a classification setting where
class labels are known for each instance: distances between points in the
same class can be constrained as similar, and points in different classes
can be constrained as dissimilar.

Given a set of inter-point distance constraints as described above, our
problem is to learn a positive-definite matrix $A$ that parameterizes the
corresponding Mahalanobis distance \eqref{eq:1}. Typically, this learned
distance function is used to improve the accuracy of a $k$-nearest neighbor
classifier, or to incorporate semi-supervision into a distance-based clustering
algorithm.  In many settings, prior information about the Mahalanobis
distance function itself is known.  In settings where data is Gaussian,
parameterizing the distance function by the inverse of the
sample covariance may be appropriate.  In other domains, squared Euclidean
distance (i.e. the Mahalanobis distance corresponding to the identity
matrix) may work well empirically.   Thus, we regularize the Mahalanobis matrix
$A$ to be as close as possible to a given Mahalanobis distance function,
parameterized by $A_0$.   

We now quantify the measure of ``closeness'' between $A$ and $A_0$ via
a natural information-theoretic approach.  There exists a simple
bijection (up to a scaling function) between the set of Mahalanobis
distances and the set of equal-mean multivariate Gaussian
distributions (without loss of generality, we can assume the Gaussians
have mean $\bm{\mu}$).  Given a Mahalanobis distance parameterized by
$A$, we express its corresponding multivariate Gaussian as
$p(\bm{x};A) = \frac{1}{Z}\exp{(-\frac{1}{2}d_{A}(\bm{x},
\bm{\mu}))}$, where $Z$ is a normalizing constant and $A^{-1}$ is the
covariance of the distribution.  Using this bijection, we measure the
distance between two Mahalanobis distance functions parameterized by
$A_0$ and $A$ by the (differential) relative entropy between their
corresponding multivariate Gaussians:
\begin{equation}
  \label{eq:re}
  %\begin{split}
  \hskip -12pt\KL(p(\bm{x}; A_o) \| p(\bm{x}; A))
    = \int p(\bm{x}; A_0) \log \frac{p(\bm{x}; A_0)}{p(\bm{x};
       A)}\, d \bm{x}. 
   %\end{split}
\end{equation}
The distance \eqref{eq:re} provides a well-founded measure of ``closeness''
between two Mahalanobis distance functions and forms the basis of our
problem given below.

Given pairs of similar points $S$ and pairs of dissimilar points $D$,
our distance metric learning problem is 
\begin{equation}
  \label{eq:obj}
  \begin{split}
    \min_{A}\quad &\KL(p(\bm{x}; A_0) \| p(\bm{x}; A))  \\
    \text{subject to}\quad & \dist (\bm{x}_i, \bm{x}_j) \leq u \qquad
    (i,j) \in S, \\
    & \dist (\bm{x}_i, \bm{x}_j) \geq \ell \qquad\  (i,j) \in D.
  \end{split}
\end{equation}

In the above formulation, we consider simple distance constraints for similar
and dissimilar points; however, it is straightforward to incorporate other
constraints.  For example,~\cite{joachim} consider a formulation where the
distance metric is learned subject to relative nearness constraints (as in,
the distance between $i$ and $j$ is closer than the distance between $i$ and
$k$). Our approach can be easily adapted to handle this setting.  In fact, it
is possible to incorporate arbitrary linear constraints into our framework in
a straightforward manner.  For simplicity, we present the algorithm under the
simple distance constraints given above.  

% Also note that when $A_0 = I$,
% (\ref{eq:obj}) may be viewed as seeking the Gaussian with maximum
% (differential) entropy subject to the constraints.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

